Provable Certificates for Adversarial Examples: Fitting a Ball in the Union of Polytopes

We propose a novel method for computing exact pointwise robustness of deep neural networks for all convex $\ell_p$ norms. Our algorithm, GeoCert, finds the largest $\ell_p$ ball centered at an input point $x_0$, within which the output class of a given neural network with ReLU nonlinearities remains unchanged. We relate the problem of computing pointwise robustness of these networks to that of computing the maximum norm ball with a fixed center that can be contained in a non-convex polytope. This is a challenging problem in general, however we show that there exists an efficient algorithm to compute this for polyhedral complices. Further we show that piecewise linear neural networks partition the input space into a polyhedral complex. Our algorithm has the ability to almost immediately output a nontrivial lower bound to the pointwise robustness which is iteratively improved until it ultimately becomes tight. We empirically show that our approach generates distance lower bounds that are tighter compared to prior work, under moderate time constraints.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> references.tex <==
@BOOK{Schrijver1998-em,
  title     = "Theory of Linear and Integer Programming",
  author    = "Schrijver, Alexander",
  abstract  = "Theory of Linear and Integer Programming Alexander Schrijver
               Centrum voor Wiskunde en Informatica, Amsterdam, The Netherlands
               This book describes the theory of linear and integer programming
               and surveys the algorithms for linear and integer programming
               problems, focusing on complexity analysis. It aims at
               complementing the more practically oriented books in this field.
               A special feature is the author's coverage of important recent
               developments in linear and integer programming. Applications to
               combinatorial optimization are given, and the author also
               includes extensive historical surveys and bibliographies. The
               book is intended for graduate students and researchers in
               operations research, mathematics and computer science. It will
               also be of interest to mathematical historians. Contents 1
               Introduction and preliminaries; 2 Problems, algorithms, and
               complexity; 3 Linear algebra and complexity; 4 Theory of
               lattices and linear diophantine equations; 5 Algorithms for
               linear diophantine equations; 6 Diophantine approximation and
               basis reduction; 7 Fundamental concepts and results on
               polyhedra, linear inequalities, and linear programming; 8 The
               structure of polyhedra; 9 Polarity, and blocking and
               anti-blocking polyhedra; 10 Sizes and the theoretical complexity
               of linear inequalities and linear programming; 11 The simplex
               method; 12 Primal-dual, elimination, and relaxation methods; 13
               Khachiyan's method for linear programming; 14 The ellipsoid
               method for polyhedra more generally; 15 Further polynomiality
               results in linear programming; 16 Introduction to integer linear
               programming; 17 Estimates in integer linear programming; 18 The
               complexity of integer linear programming; 19 Totally unimodular
               matrices: fundamental properties and examples; 20 Recognizing
               total unimodularity; 21 Further theory related to total
               unimodularity; 22 Integral polyhedra and total dual integrality;
               23 Cutting planes; 24 Further methods in integer linear
               programming; Historical and further notes on integer linear
               programming; References; Notation index; Author index; Subject
               index",
  publisher = "John Wiley \& Sons",
  month     =  jul,
  year      =  1998,
  keywords  = "geocert\_citations",
  language  = "en"
}

@BOOK{Ziegler1995-fl,
  title     = "Lectures on Polytopes",
  author    = "Ziegler, G{\"u}nter M",
  publisher = "Springer-Verlag New York",
  series    = "Graduate Texts in Mathematics",
  edition   =  1,
  year      =  1995,
  keywords  = "geocert\_citations"
}

@ARTICLE{Telgen1983-dl,
  title     = "Identifying Redundant Constraints and Implicit Equalities in
               Systems of Linear Constraints",
  author    = "Telgen, Jan",
  abstract  = "[Redundant constraints are constraints that can be omitted from
               a system of linear constraints without changing the feasible
               region. Implicit equalities are inequality constraints that can
               be replaced by equalities without changing the feasible region.
               We prove some theorems concerning the identification of both
               kinds of constraints. Based on these theorems two methods are
               developed that allow identification of all redundant constraints
               and all implicit equalities. Computational experience on small
               problems indicates a behavior at least competitive with other
               methods in this field.]",
  journal   = "Manage. Sci.",
  publisher = "INFORMS",
  volume    =  29,
  number    =  10,
  pages     = "1209--1222",
  year      =  1983,
  keywords  = "geocert\_citations"
}

@ARTICLE{Raghunathan2018-nu,
  title         = "Certified Defenses against Adversarial Examples",
  author        = "Raghunathan, Aditi and Steinhardt, Jacob and Liang, Percy",
  abstract      = "While neural networks have achieved high accuracy on
                   standard image classification benchmarks, their accuracy
                   drops to nearly zero in the presence of small adversarial
                   perturbations to test inputs. Defenses based on
                   regularization and adversarial training have been proposed,
                   but often followed by new, stronger attacks that defeat
                   these defenses. Can we somehow end this arms race? In this
                   work, we study this problem for neural networks with one
                   hidden layer. We first propose a method based on a
                   semidefinite relaxation that outputs a certificate that for
                   a given network and test input, no attack can force the
                   error to exceed a certain value. Second, as this certificate
                   is differentiable, we jointly optimize it with the network
                   parameters, providing an adaptive regularizer that
                   encourages robustness against all attacks. On MNIST, our
                   approach produces a network and a certificate that no attack
                   that perturbs each pixel by at most \textbackslashepsilon =
                   0.1 can cause more than 35\% test error.",
  month         =  jan,
  year          =  2018,
  keywords      = "geocert\_citations",
  archivePrefix = "arXiv",
  primaryClass  = "cs.LG",
  eprint        = "1801.09344"
}

% The entry below contains non-ASCII chars that could not be converted
% to a LaTeX equivalent.
@ARTICLE{Cao_undated-af,
  title    = "Mitigating Evasion Aacks to Deep Neural Networks via
              Region-based Classification",
  author   = "Cao, Xiaoyu and Gong, Neil Zhenqiang",
  keywords = "geocert\_citations"
}

@ARTICLE{Sinha_undated-rq,
  title    = "{CERTIFYING} {SOME} {DISTRIBUTIONAL} {ROBUSTNESS} {WITH}
              {PRINCIPLED} {ADVERSARIAL} {TRAINING}",
  author   = "Sinha, Aman and Namkoong, Hongseok and Duchi, John",
  keywords = "geocert\_citations"
}

@ARTICLE{Ruppert1992-ko,
  title    = "On the difficulty of triangulating three-dimensional Nonconvex
              Polyhedra",
  author   = "Ruppert, Jim and Seidel, Raimund",
  abstract = "A number of different polyhedraldecomposition problems have
              previously been studied, most notably the problem of
              triangulating a simple polygon. We are concerned with
              thepolyhedron triangulation problem: decomposing a
              three-dimensional polyhedron into a set of nonoverlapping
              tetrahedra whose vertices must be vertices of the polyhedron. It
              has previously been shown that some polyhedra cannot be
              triangulated in this fashion. We show that the problem of
              deciding whether a given polyhedron can be triangulated is
              NP-complete, and hence likely to be computationally intractable.
              The problem remains NP-complete when restricted to the case of
              star-shaped polyhedra. Various versions of the question of how
              many Steiner points are needed to triangulate a polyhedron also
              turn out to be NP-hard.",
  journal  = "Discrete Comput. Geom.",
  volume   =  7,
  number   =  3,
  pages    = "227--253",
  month    =  mar,
  year     =  1992,
  keywords = "geocert\_citations"
}

@ARTICLE{Cheng2017-xq,
  title         = "Maximum Resilience of Artificial Neural Networks",
  author        = "Cheng, Chih-Hong and N{\"u}hrenberg, Georg and Ruess, Harald",
  abstract      = "The deployment of Artificial Neural Networks (ANNs) in
                   safety-critical applications poses a number of new
                   verification and certification challenges. In particular,
                   for ANN-enabled self-driving vehicles it is important to
                   establish properties about the resilience of ANNs to noisy
                   or even maliciously manipulated sensory input. We are
                   addressing these challenges by defining resilience
                   properties of ANN-based classifiers as the maximal amount of
                   input or sensor perturbation which is still tolerated. This
                   problem of computing maximal perturbation bounds for ANNs is
                   then reduced to solving mixed integer optimization problems
                   (MIP). A number of MIP encoding heuristics are developed for
                   drastically reducing MIP-solver runtimes, and using
                   parallelization of MIP-solvers results in an almost linear
                   speed-up in the number (up to a certain limit) of computing
                   cores in our experiments. We demonstrate the effectiveness
                   and scalability of our approach by means of computing
                   maximal resilience bounds for a number of ANN benchmark sets
                   ranging from typical image recognition scenarios to the
                   autonomous maneuvering of robots.",
  month         =  apr,
  year          =  2017,
  keywords      = "Adversarial Examples;geocert\_citations",
  archivePrefix = "arXiv",
  primaryClass  = "cs.LG",
  eprint        = "1705.01040"
}

@ARTICLE{Ehlers2017-pg,
  title         = "Formal Verification of {Piece-Wise} Linear {Feed-Forward}
                   Neural Networks",
  author        = "Ehlers, Ruediger",
  abstract      = "We present an approach for the verification of feed-forward
                   neural networks in which all nodes have a piece-wise linear
                   activation function. Such networks are often used in deep
                   learning and have been shown to be hard to verify for modern
                   satisfiability modulo theory (SMT) and integer linear
                   programming (ILP) solvers. The starting point of our
                   approach is the addition of a global linear approximation of
                   the overall network behavior to the verification problem
                   that helps with SMT-like reasoning over the network
                   behavior. We present a specialized verification algorithm
                   that employs this approximation in a search process in which
                   it infers additional node phases for the non-linear nodes in
                   the network from partial node phase assignments, similar to
                   unit propagation in classical SAT solving. We also show how
                   to infer additional conflict clauses and safe node fixtures
                   from the results of the analysis steps performed during the
                   search. The resulting approach is evaluated on collision
                   avoidance and handwritten digit recognition case studies.",
  month         =  may,
  year          =  2017,
  keywords      = "Adversarial Examples;geocert\_citations",
  archivePrefix = "arXiv",
  primaryClass  = "cs.LO",
  eprint        = "1705.01320"
}

@ARTICLE{Katz2017-qz,
  title         = "Reluplex: An Efficient {SMT} Solver for Verifying Deep
                   Neural Networks",
  author        = "Katz, Guy and Barrett, Clark and Dill, David and Julian,
                   Kyle and Kochenderfer, Mykel",
  abstract      = "Deep neural networks have emerged as a widely used and
                   effective means for tackling complex, real-world problems.
                   However, a major obstacle in applying them to
                   safety-critical systems is the great difficulty in providing
                   formal guarantees about their behavior. We present a novel,
                   scalable, and efficient technique for verifying properties
                   of deep neural networks (or providing counter-examples). The
                   technique is based on the simplex method, extended to handle
                   the non-convex Rectified Linear Unit (ReLU) activation
                   function, which is a crucial ingredient in many modern
                   neural networks. The verification procedure tackles neural
                   networks as a whole, without making any simplifying
                   assumptions. We evaluated our technique on a prototype deep
                   neural network implementation of the next-generation
                   airborne collision avoidance system for unmanned aircraft
                   (ACAS Xu). Results show that our technique can successfully
                   prove properties of networks that are an order of magnitude
                   larger than the largest networks verified using existing
                   methods.",
  month         =  feb,
  year          =  2017,
  keywords      = "Adversarial Examples;geocert\_citations",
  archivePrefix = "arXiv",
  primaryClass  = "cs.AI",
  eprint        = "1702.01135"
}

@ARTICLE{Zhang2018-fl,
  title         = "Efficient Neural Network Robustness Certification with
                   General Activation Functions",
  author        = "Zhang, Huan and Weng, Tsui-Wei and Chen, Pin-Yu and Hsieh,
                   Cho-Jui and Daniel, Luca",
  abstract      = "Finding minimum distortion of adversarial examples and thus
                   certifying robustness in neural network classifiers for
                   given data points is known to be a challenging problem.
                   Nevertheless, recently it has been shown to be possible to
                   give a non-trivial certified lower bound of minimum
                   adversarial distortion, and some recent progress has been
                   made towards this direction by exploiting the piece-wise
                   linear nature of ReLU activations. However, a generic
                   robustness certification for general activation functions
                   still remains largely unexplored. To address this issue, in
                   this paper we introduce CROWN, a general framework to
                   certify robustness of neural networks with general
                   activation functions for given input data points. The
                   novelty in our algorithm consists of bounding a given
                   activation function with linear and quadratic functions,
                   hence allowing it to tackle general activation functions
                   including but not limited to four popular choices: ReLU,
                   tanh, sigmoid and arctan. In addition, we facilitate the
                   search for a tighter certified lower bound by adaptively
                   selecting appropriate surrogates for each neuron activation.
                   Experimental results show that CROWN on ReLU networks can
                   notably improve the certified lower bounds compared to the
                   current state-of-the-art algorithm Fast-Lin, while having
                   comparable computational efficiency. Furthermore, CROWN also
                   demonstrates its effectiveness and flexibility on networks
                   with general activation functions, including tanh, sigmoid
                   and arctan.",
  month         =  nov,
  year          =  2018,
  keywords      = "Adversarial Examples;geocert\_citations",
  archivePrefix = "arXiv",
  primaryClass  = "cs.LG",
  eprint        = "1811.00866"
}

@ARTICLE{Ehmann2001-ij,
  title    = "Accurate and Fast Proximity Queries Between Polyhedra Using
              Convex Surface Decomposition",
  author   = "Ehmann, Stephen A and Lin, Ming C",
  abstract = "The need to perform fast and accurate proximity queries arises
              frequently in physically-based modeling, simulation, animation,
              real-time interaction within a virtual environment, and game
              dynamics. The set of proximity queries include intersection
              detection, tolerance verification, exact and approximate minimum
              distance computation, and (disjoint) contact determination.
              Specialized data structures and algorithms have often been
              designed to perform each type of query separately. We present a
              unified approach to perform any of these queries seamlessly for
              general, rigid polyhedral objects with boundary representations
              which are orientable 2-manifolds. The proposed method involves a
              hierarchical data structure built upon a surface decomposition of
              the models. Furthermore, the incremental query algorithm takes
              advantage of coherence between successive frames. It has been
              applied to complex benchmarks and compares very favorably with
              earlier algorithms and systems.",
  journal  = "Comput. Graph. Forum",
  volume   =  20,
  number   =  3,
  pages    = "500--511",
  month    =  sep,
  year     =  2001,
  keywords = "Adversarial Examples;geocert\_citations"
}

@ARTICLE{Pang2017-wl,
  title         = "Towards Robust Detection of Adversarial Examples",
  author        = "Pang, Tianyu and Du, Chao and Dong, Yinpeng and Zhu, Jun",
  abstract      = "Although the recent progress is substantial, deep learning
                   methods can be vulnerable to the maliciously generated
                   adversarial examples. In this paper, we present a novel
                   training procedure and a thresholding test strategy, towards
                   robust detection of adversarial examples. In training, we
                   propose to minimize the reverse cross-entropy (RCE), which
                   encourages a deep network to learn latent representations
                   that better distinguish adversarial examples from normal
                   ones. In testing, we propose to use a thresholding strategy
                   as the detector to filter out adversarial examples for
                   reliable predictions. Our method is simple to implement
                   using standard algorithms, with little extra training cost
                   compared to the common cross-entropy minimization. We apply
                   our method to defend various attacking methods on the widely
                   used MNIST and CIFAR-10 datasets, and achieve significant
                   improvements on robust predictions under all the threat
                   models in the adversarial setting.",
  month         =  jun,
  year          =  2017,
  keywords      = "Adversarial Examples;geocert\_citations",
  archivePrefix = "arXiv",
  primaryClass  = "cs.LG",
  eprint        = "1706.00633"
}

@INCOLLECTION{Wong2018-gw,
  title     = "Scaling provable adversarial defenses",
  booktitle = "Advances in Neural Information Processing Systems 31",
  author    = "Wong, Eric and Schmidt, Frank and Metzen, Jan Hendrik and
               Kolter, J Zico",
  editor    = "Bengio, S and Wallach, H and Larochelle, H and Grauman, K and
               Cesa-Bianchi, N and Garnett, R",
  publisher = "Curran Associates, Inc.",
  pages     = "8409--8418",
  year      =  2018,
  keywords  = "NIPS18 AEs;Adversarial Examples;geocert\_citations;NeurIPS18 AEs"
}

@ARTICLE{Xiao2018-aj,
  title         = "Training for Faster Adversarial Robustness Verification via
                   Inducing {ReLU} Stability",
  author        = "Xiao, Kai Y and Tjeng, Vincent and Shafiullah, Nur Muhammad
                   and Madry, Aleksander",
  abstract      = "We explore the concept of co-design in the context of neural
                   network verification. Specifically, we aim to train deep
                   neural networks that not only are robust to adversarial
                   perturbations but also whose robustness can be verified more
                   easily. To this end, we identify two properties of network
                   models - weight sparsity and so-called ReLU stability - that
                   turn out to significantly impact the complexity of the
                   corresponding verification task. We demonstrate that
                   improving weight sparsity alone already enables us to turn
                   computationally intractable verification problems into
                   tractable ones. Then, improving ReLU stability leads to an
                   additional 4-13x speedup in verification times. An important
                   feature of our methodology is its ``universality,'' in the
                   sense that it can be used with a broad range of training
                   procedures and verification approaches.",
  month         =  sep,
  year          =  2018,
  keywords      = "Adversarial Examples;geocert\_citations",
  archivePrefix = "arXiv",
  primaryClass  = "cs.LG",
  eprint        = "1809.03008"
}

@ARTICLE{Zico_Kolter2017-va,
  title         = "Provable defenses against adversarial examples via the
                   convex outer adversarial polytope",
  author        = "Zico Kolter, J and Wong, Eric",
  abstract      = "We propose a method to learn deep ReLU-based classifiers
                   that are provably robust against norm-bounded adversarial
                   perturbations (on the training data; for previously unseen
                   examples, the approach will be guaranteed to detect all
                   adversarial examples, though it may flag some
                   non-adversarial examples as well). The basic idea of the
                   approach is to consider a convex outer approximation of the
                   set of activations reachable through a norm-bounded
                   perturbation, and we develop a robust optimization procedure
                   that minimizes the worst case loss over this outer region
                   (via a linear program). Crucially, we show that the dual
                   problem to this linear program can be represented itself as
                   a deep network similar to the backpropagation network,
                   leading to very efficient optimization approaches that
                   produce guaranteed bounds on the robust loss. The end result
                   is that by executing a few more forward and backward passes
                   through a slightly modified version of the original network
                   (though possibly with much larger batch sizes), we can learn
                   a classifier that is provably robust to any norm-bounded
                   adversarial attack. We illustrate the approach on a toy 2D
                   robust classification task, and on a simple convolutional
                   architecture applied to MNIST, where we produce a classifier
                   that provably has less than 8.4\% test error for any
                   adversarial attack with bounded $\ell_\infty$ norm less than
                   $\epsilon = 0.1$. This represents the largest verified
                   network that we are aware of, and we discuss future
                   challenges in scaling the approach to much larger domains.",
  month         =  nov,
  year          =  2017,
  keywords      = "Adversarial Examples;geocert\_citations",
  archivePrefix = "arXiv",
  primaryClass  = "cs.LG",
  eprint        = "1711.00851"
}

@ARTICLE{Hein2017-ky,
  title         = "Formal Guarantees on the Robustness of a Classifier against
                   Adversarial Manipulation",
  author        = "Hein, Matthias and Andriushchenko, Maksym",
  abstract      = "Recent work has shown that state-of-the-art classifiers are
                   quite brittle, in the sense that a small adversarial change
                   of an originally with high confidence correctly classified
                   input leads to a wrong classification again with high
                   confidence. This raises concerns that such classifiers are
                   vulnerable to attacks and calls into question their usage in
                   safety-critical systems. We show in this paper for the first
                   time formal guarantees on the robustness of a classifier by
                   giving instance-specific lower bounds on the norm of the
                   input manipulation required to change the classifier
                   decision. Based on this analysis we propose the
                   Cross-Lipschitz regularization functional. We show that
                   using this form of regularization in kernel methods resp.
                   neural networks improves the robustness of the classifier
                   without any loss in prediction performance.",
  month         =  may,
  year          =  2017,
  keywords      = "Adversarial Examples;geocert\_citations;Unsup final
                   project;Adversarial Examples (DG)",
  archivePrefix = "arXiv",
  primaryClass  = "cs.LG",
  eprint        = "1705.08475"
}



@ARTICLE{Bastani2016-zs,
  title         = "Measuring Neural Net Robustness with Constraints",
  author        = "Bastani, Osbert and Ioannou, Yani and Lampropoulos, Leonidas
                   and Vytiniotis, Dimitrios and Nori, Aditya and Criminisi,
                   Antonio",
  abstract      = "Despite having high accuracy, neural nets have been shown to
                   be susceptible to adversarial examples, where a small
                   perturbation to an input can cause it to become mislabeled.
                   We propose metrics for measuring the robustness of a neural
                   net and devise a novel algorithm for approximating these
                   metrics based on an encoding of robustness as a linear
                   program. We show how our metrics can be used to evaluate the
                   robustness of deep neural nets with experiments on the MNIST
                   and CIFAR-10 datasets. Our algorithm generates more
                   informative estimates of robustness metrics compared to
                   estimates based on existing algorithms. Furthermore, we show
                   how existing approaches to improving robustness ``overfit''
                   to adversarial examples generated using a specific
                   algorithm. Finally, we show that our techniques can be used
                   to additionally improve neural net robustness both according
                   to the metrics that we propose, but also according to
                   previously proposed metrics.",
  month         =  may,
  year          =  2016,
  archivePrefix = "arXiv",
  primaryClass  = "cs.LG",
  eprint        = "1605.07262"
}



@ARTICLE{Tjeng2017-qp,
  title         = "Evaluating Robustness of Neural Networks with Mixed Integer
                   Programming",
  author        = "Tjeng, Vincent and Xiao, Kai and Tedrake, Russ",
  abstract      = "Neural networks have demonstrated considerable success on a
                   wide variety of real-world problems. However, networks
                   trained only to optimize for training accuracy can often be
                   fooled by adversarial examples - slightly perturbed inputs
                   that are misclassified with high confidence. Verification of
                   networks enables us to gauge their vulnerability to such
                   adversarial examples. We formulate verification of
                   piecewise-linear neural networks as a mixed integer program.
                   On a representative task of finding minimum adversarial
                   distortions, our verifier is two to three orders of
                   magnitude quicker than the state-of-the-art. We achieve this
                   computational speedup via tight formulations for
                   non-linearities, as well as a novel presolve algorithm that
                   makes full use of all information available. The
                   computational speedup allows us to verify properties on
                   convolutional networks with an order of magnitude more ReLUs
                   than networks previously verified by any complete verifier.
                   In particular, we determine for the first time the exact
                   adversarial accuracy of an MNIST classifier to perturbations
                   with bounded $l_\infty$ norm $\epsilon=0.1$: for this
                   classifier, we find an adversarial example for 4.38\% of
                   samples, and a certificate of robustness (to perturbations
                   with bounded norm) for the remainder. Across all robust
                   training procedures and network architectures considered, we
                   are able to certify more samples than the state-of-the-art
                   and find more adversarial examples than a strong first-order
                   attack.",
  month         =  nov,
  year          =  2017,
  archivePrefix = "arXiv",
  primaryClass  = "cs.LG",
  eprint        = "1711.07356"
}



@ARTICLE{Krishnamurthy2018-ow,
  title         = "A Dual Approach to Scalable Verification of Deep Networks",
  author        = "{Krishnamurthy} and {Dvijotham} and Stanforth, Robert and
                   Gowal, Sven and Mann, Timothy and Kohli, Pushmeet",
  abstract      = "This paper addresses the problem of formally verifying
                   desirable properties of neural networks, i.e., obtaining
                   provable guarantees that neural networks satisfy
                   specifications relating their inputs and outputs (robustness
                   to bounded norm adversarial perturbations, for example).
                   Most previous work on this topic was limited in its
                   applicability by the size of the network, network
                   architecture and the complexity of properties to be
                   verified. In contrast, our framework applies to a general
                   class of activation functions and specifications on neural
                   network inputs and outputs. We formulate verification as an
                   optimization problem (seeking to find the largest violation
                   of the specification) and solve a Lagrangian relaxation of
                   the optimization problem to obtain an upper bound on the
                   worst case violation of the specification being verified.
                   Our approach is anytime i.e. it can be stopped at any time
                   and a valid bound on the maximum violation can be obtained.
                   We develop specialized verification algorithms with provable
                   tightness guarantees under special assumptions and
                   demonstrate the practical significance of our general
                   verification approach on a variety of verification tasks.",
  month         =  mar,
  year          =  2018,
  archivePrefix = "arXiv",
  primaryClass  = "cs.LG",
  eprint        = "1803.06567"
}


@INPROCEEDINGS{Mirman2018-nx,
  title     = "Differentiable Abstract Interpretation for Provably Robust
               Neural Networks",
  booktitle = "Proceedings of the 35th International Conference on Machine
               Learning",
  author    = "Mirman, Matthew and Gehr, Timon and Vechev, Martin",
  editor    = "Dy, Jennifer and Krause, Andreas",
  abstract  = "We introduce a scalable method for training robust neural
               networks based on abstract interpretation. We present several
               abstract transformers which balance efficiency with precision
               and show these can be used to train large neural networks that
               are certifiably robust to adversarial perturbations.",
  publisher = "PMLR",
  volume    =  80,
  pages     = "3578--3586",
  series    = "Proceedings of Machine Learning Research",
  year      =  2018,
  address   = "Stockholmsm{\"a}ssan, Stockholm Sweden"
}




@ARTICLE{Tsuzuku2018-nx,
  title         = "{Lipschitz-Margin} Training: Scalable Certification of
                   Perturbation Invariance for Deep Neural Networks",
  author        = "Tsuzuku, Yusuke and Sato, Issei and Sugiyama, Masashi",
  abstract      = "High sensitivity of neural networks against malicious
                   perturbations on inputs causes security concerns. To take a
                   steady step towards robust classifiers, we aim to create
                   neural network models provably defended from perturbations.
                   Prior certification work requires strong assumptions on
                   network structures and massive computational costs, and thus
                   the range of their applications was limited. From the
                   relationship between the Lipschitz constants and prediction
                   margins, we present a computationally efficient calculation
                   technique to lower-bound the size of adversarial
                   perturbations that can deceive networks, and that is widely
                   applicable to various complicated networks. Moreover, we
                   propose an efficient training procedure that robustifies
                   networks and significantly improves the provably guarded
                   areas around data points. In experimental evaluations, our
                   method showed its ability to provide a non-trivial guarantee
                   and enhance robustness for even large networks.",
  month         =  feb,
  year          =  2018,
  archivePrefix = "arXiv",
  primaryClass  = "cs.CV",
  eprint        = "1802.04034"
}



@ARTICLE{Szegedy2013-yt,
  title         = "Intriguing properties of neural networks",
  author        = "Szegedy, Christian and Zaremba, Wojciech and Sutskever, Ilya
                   and Bruna, Joan and Erhan, Dumitru and Goodfellow, Ian and
                   Fergus, Rob",
  abstract      = "Deep neural networks are highly expressive models that have
                   recently achieved state of the art performance on speech and
                   visual recognition tasks. While their expressiveness is the
                   reason they succeed, it also causes them to learn
                   uninterpretable solutions that could have counter-intuitive
                   properties. In this paper we report two such properties.
                   First, we find that there is no distinction between
                   individual high level units and random linear combinations
                   of high level units, according to various methods of unit
                   analysis. It suggests that it is the space, rather than the
                   individual units, that contains of the semantic information
                   in the high layers of neural networks. Second, we find that
                   deep neural networks learn input-output mappings that are
                   fairly discontinuous to a significant extend. We can cause
                   the network to misclassify an image by applying a certain
                   imperceptible perturbation, which is found by maximizing the
                   network's prediction error. In addition, the specific nature
                   of these perturbations is not a random artifact of learning:
                   the same perturbation can cause a different network, that
                   was trained on a different subset of the dataset, to
                   misclassify the same input.",
  month         =  dec,
  year          =  2013,
  archivePrefix = "arXiv",
  primaryClass  = "cs.CV",
  eprint        = "1312.6199"
}



@BOOK{Boyd2004-dj,
  title     = "Convex Optimization",
  author    = "Boyd, Stephen and Vandenberghe, Lieven",
  abstract  = "Convex optimization problems arise frequently in many different
               fields. This book provides a comprehensive introduction to the
               subject, and shows in detail how such problems can be solved
               numerically with great efficiency. The book begins with the
               basic elements of convex sets and functions, and then describes
               various classes of convex optimization problems. Duality and
               approximation techniques are then covered, as are statistical
               estimation techniques. Various geometrical problems are then
               presented, and there is detailed discussion of unconstrained and
               constrained minimization problems, and interior-point methods.
               The focus of the book is on recognizing convex optimization
               problems and then finding the most appropriate technique for
               solving them. It contains many worked examples and homework
               exercises and will appeal to students, researchers and
               practitioners in fields such as engineering, computer science,
               mathematics, statistics, finance and economics.",
  publisher = "Cambridge University Press",
  month     =  mar,
  year      =  2004,
  language  = "en"
}


@ARTICLE{Botkin1994-ln,
  title     = "An algorithm for finding the Chebyshev center of a convex
               polyhedron",
  author    = "Botkin, N D and Turova-Botkina, V L",
  abstract  = "An algorithm for finding the Chebyshev center of a finite point
               set in the Euclidean spaceRnis proposed. The algorithm
               terminates after a finite number of iterations. In each
               iteration of the algorithm the current point is projected
               orthogonally onto the convex hull of a subset of the given point
               set.",
  journal   = "Appl. Math. Optim.",
  publisher = "Springer",
  volume    =  29,
  number    =  2,
  pages     = "211--222",
  month     =  mar,
  year      =  1994
}



% The entry below contains non-ASCII chars that could not be converted
% to a LaTeX equivalent.
@ARTICLE{Karmarkar1984-ah,
  title    = "A new polynomial-time algorithm for linear programming",
  author   = "Karmarkar, N",
  abstract = "We present a new polynomial-time algorithm for linear
              programming. In the worst case, the algorithm requiresO(n3.5L)
              arithmetic operations onO(L) bit numbers, wheren is the number of
              variables andL is the number of bits in the input. The
              running-time of this algorithm is better than the ellipsoid
              algorithm by a factor ofO(n2.5). We prove that given a polytopeP
              and a strictly interior point a $\epsilon$P, there is a
              projective transformation of the space that mapsP, a toP′, a′
              having the following property. The ratio of the radius of the
              smallest sphere with center a′, containingP′ to the radius of the
              largest sphere with center a′ contained inP′ isO(n). The
              algorithm consists of repeated application of such projective
              transformations each followed by optimization over an inscribed
              sphere to create a sequence of points which converges to the
              optimal solution in polynomial time.",
  journal  = "Combinatorica",
  volume   =  4,
  number   =  4,
  pages    = "373--395",
  month    =  dec,
  year     =  1984
}



@ARTICLE{Ye1989-ri,
  title    = "An extension of Karmarkar's projective algorithm for convex
              quadratic programming",
  author   = "Ye, Yinyu and Tse, Edison",
  abstract = "We present an extension of Karmarkar's linear programming
              algorithm for solving a more general group of optimization
              problems: convex quadratic programs. This extension is based on
              the iterated application of the objective augmentation and the
              projective transformation, followed by optimization over an
              inscribing ellipsoid centered at the current solution. It creates
              a sequence of interior feasible points that converge to the
              optimal feasible solution in O(Ln) iterations; each iteration can
              be computed in O(Ln3) arithmetic operations, wheren is the number
              of variables andL is the number of bits in the input. In this
              paper, we emphasize its convergence property, practical
              efficiency, and relation to the ellipsoid method.",
  journal  = "Math. Program.",
  volume   =  44,
  number   =  1,
  pages    = "157--179",
  month    =  may,
  year     =  1989
}


% The entry below contains non-ASCII chars that could not be converted
% to a LaTeX equivalent.
@ARTICLE{Stanley2004-qv,
  title     = "An introduction to hyperplane arrangements",
  author    = "Stanley, Richard P",
  abstract  = "Page numbers refer to the page numbers at the top of the pages,
               not to the page count of the PDF file.• page 2: You speak of the
               ``usual dot product'', but there is no ``usual dot product'' on
               a general finite-dimensional K-vector space. If you want to work
               in this generality, you should …",
  journal   = "Geometric combinatorics",
  publisher = "cip.ifi.lmu.de",
  volume    =  13,
  pages     = "389--496",
  year      =  2004
}



@ARTICLE{Chazelle1997-hl,
  title    = "Decomposing the boundary of a nonconvex polyhedron",
  author   = "Chazelle, B and Palios, L",
  abstract = "We show that the boundary of a three-dimensional polyhedron withr
              reflex angles and arbitrary genus can be subdivided intoO(r)
              connected pieces, each of which lies on the boundary of its
              convex hull. A remarkable feature of this result is that the
              number of these convex-like pieces is independent of the number
              of vertices. Furthermore, it is linear inr, which contrasts with
              a quadratic worst-case lower bound in the number of convex pieces
              needed to decompose the polyhedron itself. The number of new
              vertices introduced in the process isO(n). The decomposition can
              be computed inO(n+rlogr) time.",
  journal  = "Algorithmica",
  volume   =  17,
  number   =  3,
  pages    = "245--265",
  month    =  mar,
  year     =  1997
}




@ARTICLE{Goodfellow2014-vh,
  title         = "Explaining and Harnessing Adversarial Examples",
  author        = "Goodfellow, Ian J and Shlens, Jonathon and Szegedy,
                   Christian",
  abstract      = "Several machine learning models, including neural networks,
                   consistently misclassify adversarial examples---inputs
                   formed by applying small but intentionally worst-case
                   perturbations to examples from the dataset, such that the
                   perturbed input results in the model outputting an incorrect
                   answer with high confidence. Early attempts at explaining
                   this phenomenon focused on nonlinearity and overfitting. We
                   argue instead that the primary cause of neural networks'
                   vulnerability to adversarial perturbation is their linear
                   nature. This explanation is supported by new quantitative
                   results while giving the first explanation of the most
                   intriguing fact about them: their generalization across
                   architectures and training sets. Moreover, this view yields
                   a simple and fast method of generating adversarial examples.
                   Using this approach to provide examples for adversarial
                   training, we reduce the test set error of a maxout network
                   on the MNIST dataset.",
  month         =  dec,
  year          =  2014,
  archivePrefix = "arXiv",
  primaryClass  = "stat.ML",
  eprint        = "1412.6572"
}

